Long-term Value of Flexibility from Flexible Assets in Building Operation

In this work, we investigate how flexible assets within a residential building influence the long-term impact of operation. We use a measured-peak grid tariff (MPGT) that puts a cost on the highest single-hour peak import over the month. We apply a mathematical model of a Home Energy Management System (HEMS) together with Stochastic Dynamic Programming (SDP), which calculates the long-term impact of operating as a non-linear expected future cost curve (EFCC) from the end of the scheduling period to the start. The proposed model is applied to a case study for a Norwegian building with smart control of a battery energy storage system (BESS), Electric vehicle (EV) charging and space heating (SH). Each of the flexible assets are investigated individually with MPGT and for an energy-based grid tariff. The results showed that EV charging has the highest peak-power impact in the system, decreasing the total electricity cost by 14.6% with MPGT when controllable compared to a reference case with passive charging. It is further shown how the EFCC helps achieve optimal timing and level of the peak demand, where it co-optimizes both real-time pricing and the MPGT.

==> chapters/old_result_for_perhaps_other_work.tex <==
\subsection{Flexible performance on Electricity schemes}


\subsection{Individual performance of flexible assets} \label{Ind_flex_assets_result}

Insert good intro.

The overall overview over the economic performance of all cases are found in Table [Insert, but should it be here?].

\subsubsection{Passive building scheduling}

The overview of the SDP algorithm regarding a passive building scheduling can be found in Figures [all others] as a comparison measure for the other cases. In general, the passive strategy does not utilize any flexible assets to help control the peak import, which results in that the peak import will be set by the hour with highest peak power during the month. The EFCC for this thus has a close to vertical marginal increase from 0 to the marginal cost for the MP grid tariff. 

With a passive building structure, the flexible assets are not controlled to react on the peak import. Thus, the EV will have a charging strategy where it charges at max charger capacity until it has fully charged whenever it is not at maximum capacity, the stationary battery will not be in use, and the space heating will keep the indoor temperature at 22 $^{\circ} C$ continuously. 


\subsubsection{Stationary battery}

The EFCC when enabling the stationary battery to be flexible is shown in Figure \ref{fig:Battery_EFCC}. When comparing against the passive EFCC, the capability of the battery to load shift by storing electricity for critical hours decreases the target peak import level from day 1. For the 5 and 10 kWh battery, the target peak decreases from \textbf{8} to about \textbf{5.6} and 5.3 $\frac{kWh}{h}$, respectively. This fits with the discharge capacity of the battery, which is able to provide 2.5 kW output per hour to decrease the need for peak import. Thus, the flexibility from the battery manages to cut the peak import level in the hours needed, by charging in hours with low import and discharge in high import hours. As the battery is the only flexible asset here that has no load demand and only works to charge/discharge, it has much freedom in choosing when to operate, but also has no direct saving by rescheduling the passive behavior. This gives flexibility throughout each day and can single-handily focus its operation on lowering the total electricity cost.


\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/Batteries.png}
\caption{Plot of the EFCC for a 5 and 10 kWh stationary battery with both electricity schemes involving the MP grid tariff.}
\label{fig:Battery_EFCC}
\centering
\end{figure}



The 5 kWh battery is only capable of providing this discharge continuously for almost 2 full hours, while the 10 kWh could provide for almost 4 hours, when taking into account the efficiency losses. That the differences in target peak on both sizes are of about .4, indicates that the peak hours are not happening over prolonged periods over the month. %Thus, the low decrease in target peak from a 5 to 10 kWh battery indicated that for MP grid tariff focus, the 10 kWh battery might be over-dimensioned for this single goal.

When looking at the marginal increase of future cost for the battery sizes, that the increase is not pure vertical is influenced by two main impacts. First, the uncertainty in the problem pushes the curve more to the right side, as shown by the reference case that also have this behavior. Some scenarios need more contribution from the battery than the others. The other major impact is the efficiency losses from utilizing the battery, which is based on how much the battery needs to react. The MEFCC for the batteries are also pushed more towards the right for higher peak import, due to the efficiency savings from using the batteries less. This shows that the increasing peak import gives more flexibility in the future that adds a cost-benefit to the system. Increasing peak means that there is less need for the battery to be utilized as there is less peak to cut when necessary. This is supported by comparing the 10 kWh cases to the case without any efficiency losses, where the curve hits the peak future cost at much earlier peak import levels. The differences here is due to the efficiency loss savings that the system recovers when the battery needs to be utilized less in the future. 

When comparing the electricity schemes, one can see how the scheme with constant electricity price (F-P) has a lower marginal cost increase based on peak import level than the RT-P electricity pricing scheme for both battery sizes. The shift where F-P is lower shows how load shifting caused by the battery storage is affected on the cost of electricity. With a constant price, the timing of charging the battery is only influenced by the peak import level, and not the cost-optimal time of the day, as compared to the RT-P which also includes this factor. As the RT-P case has a higher marginal cost increase, the savings from the battery utilization is less than for the F-P. This is caused by that the RT-P manages to charge more when the electricity prices are lower than average, and thus the savings from lowering efficiency losses are lower as the electricity was cheaper to purchase. Within RT-P, the electricity price tends to be higher towards the morning and evening, which is when the battery most likely reacts to push the peak import level down, and thus would most of the time charge during off-peak hours which is when the price is lower. Thus, one can see how the F-P case charges with more expensive electricity than RT-P, which then is showcased by more efficiency savings and a lower MEFFC curve when the loss savings are primarily pushing the future cost down.

%sometimes need to charge when the electricity price is above average. This is influenced by the short-term need to charge the battery for incoming discharge opportunity, which might be only some hours in the future. Also, this could be influenced by that the RTP prices could have whole days above the average monthly price, which means that the cost for electricity is more expensive with RTP no matter the optimal time slot. However, as the opposite could be the case with RTP under average, the biggest impact comes from the short-term need for electricity and the connected efficiency losses, which indicates that the battery is utilized frequently and cannot charge all the needed energy during cheaper hours. This is also indicated by that the 10 kWh battery has a less vertical slope than the 5 kWh battery, as it can store more from low-price hours.

\subsubsection{Electric Vehicle charging}

For charging of the EV, which is only available for charging on the afternoon and during the morning, has the corresponding EFCCs shown in Figure \ref{fig:EV_EFCC_FP} and Figure \ref{fig:EV_EFCC_RTP}. As the case investigates different charger capacities, their corresponding passive EFCC is also included here. The EV needs to charge the battery before travelling to ensure safe travels, and is thus a load unit with load shifting capability.

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/EV_FP.png}
\caption{Plot of the EFCC for the EV charging with capacity of 2.3, 3.7 and 11 kW for the F-P electricity scheme.}
\label{fig:EV_EFCC_FP}
\centering
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/EV_RTP.png}
\caption{Plot of the EFCC for the EV charging with capacity of 2.3, 3.7 and 11 kW for  the RT-P electricity scheme.}
\label{fig:EV_EFCC_RTP}
\centering
\end{figure}

The first noticeable result is that all EFCC are equal when the EV charger is flexible, as their curves are atop each other. Almost regardless of the charger capacity, the EV has enough time to charge up to the optimal charging point and optimize both with and without RTP. That the curves are equal for both the F-P and RT-P cases, show that the added benefit for RTP with increasing peak is negligible. Comparing the performance against the references cases, the biggest impact there is tied to what capacity your passive EV charger has, as that pushes the peak import heavily. With a passive charger, you utilize the whole capacity, which then makes your EV charge faster, but then at the cost of higher peak power.

The flexible EV chargers have the possibility of charging for the 15 hours the EV is available, and thus has a high range of flexibility to choose when to charge. For RTP consideration, it can choose to charge during night if the evening is more power-intensive, and vice-versa, giving it room to charge outside other critical components. By this implication, the capacity of the EV charger is not critical, as the conventional 2.3 kW charger should be sufficient to fully charge it without any higher peak import impact, and as this curve is close to equal to the others, the higher capacity would not be utilized as that would push the peak import above the optimal peak level. 

The EFCC are more vertical around the critical peak power increase, mainly due to the added peak level not contributing much with the flexibility from the EV charger. This is as mentioned previously tied to the multiple hours of opportunity to charge. Also, the curve is not shifting towards the right as was the case for the stationary battery, even though the EV also has efficiency losses. This is due to the EV needing the electricity during the day, thus the charging is a must. As the EV is uni-directional, it does not change the amount it charges. The vertical curve also shows how the uncertainty regarding departure/arrival time during the month does not affect scheduling considerably, as the flexibility to react to that without any significant impact is possible.



\subsubsection{Space heating}

Space heating utilizes the heater to keep the interior temperature within the user-specified level of comfort, and this must be kept for the whole day. The EFCC performance when altering the indoor temperature boundary is shown in Figure \ref{fig:SH}. An important remark about space heating control, is that in winter days, there is a significant demand for heating to keep the indoor temperature satisfactory. Thus, the heater needs to supply thermal heat and is then diligently utilized, and the control will then mostly benefit in shifting the heating to more cost-effective hours.

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/Space_heating.png}
\caption{Plot of the EFCC for Space heating for different temperature boundaries.}
\label{fig:SH}
\centering
\end{figure}

The first observation from the EFCCs is that there is no real difference between the EFCC for the F-P and RT-P cases. This shows that the increased future cost is mostly associated with the grid tariff cost alone when comparing the two schemes as the curve is more vertical.

Another observation is that based on the temperature boundary, the optimal peak level changes. The reference case has a constant indoor temperature, which when allowing to be flexible, decreases the peak power based on the boundary given. With increasing boundary, the peak level decreases due to more flexibility in load shifting. However, one can see how the boundaries 19-25 and 20-24 have the same MEFCC, which shows that this benefit only contributes to a certain degree. With increasing boundary, one has more flexibility to shift the heating to more opportunistic hours, by increasing the temperature before high peak hours from other sources, and then resume heating after.

As mentioned, both cases 19-25 and 20-24 have equal MEFCCs, which suggests that increasing the boundary has no significant added effect on the future cost from peak import. With higher boundary, one has the capability to turn the heater off for longer duration, but the similarities here implies that the extra flexibility is not necessary to utilize to the full potential. As the dynamic properties of the state space model used for space heating increases heat losses on increasing temperature mismatch between outdoor and indoor, the optimal operating point is around the lower boundary most of the time. The heat loss difference between the two cases here are not significant as we cannot see any changes, and the boundary size does not seem to affect future cost. So the marginal losses associated with a higher lower boundary seems less significant.

For the 21-23 case, however, the lack of flexibility in indoor temperature impacts the peak level significantly. Trying to load shift heating to avoid heating during critical hours is unavoidable for the whole duration, and thus the heater must activate partly during these hours also, pushing the peak level higher. With increasing peak power, there is some value added during operation that makes the future cost a combination of grid tariff costs and added value from flexibility. However, as this curve has similar fashion to the reference case, this trend is mostly from the uncertainty, although some small changes in the lower and upper end of the curve does imply some additional benefit with the available flexibility.

\subsubsection{Summary of MEFCC analysis}

\textbf{Is this necessary?}


\subsection{Cost-effective Performance of the flexible assets}

The MEFCC described in Section \ref{Ind_flex_assets_result} gives an overview over the cost-effective strategies regarding a change in peak import levels. As the strategy includes the uncertainty of the problem, the performance is affected by this and the flexible assets capability to react. Some scenarios as shown in the MEFCCs will make the peak import level change during scheduling, as the cost-effective level would not be reachable for all scenarios. However, how much change and deviation from the initial point one can expect depends on the flexible asset, and will be covered in this analysis.

Another point is the total cost based on the flexible assets, which gives an overview over what assets contribute the most on this point.

\textbf{This is where I am currently. The figures below is the work I have finished extracting and plan to write about}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/First_check_cost.png}
\caption{Overview over expected monthly cost for the different cases for RT-P}
\label{fig:Cost_RTP}
\centering
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Pictures/First_check_peak.png}
\caption{Overview over expected ending peak for the different cases for RT-P}
\label{fig:peak_RTP}
\centering
\end{figure}


\subsubsection{Change in peak import}

\textbf{Should have a boxplot of the different cases and their performance and change in peak power.}



==> chapters/temp.tex <==
\makenomenclature

\renewcommand{\nomgroup}[1]{%
\ifthenelse{\equal{#1}{A}{\item[\textbf{SDP sets}]}{%
\ifthenelse{\equal{#1}{B}}{\item[\textbf{Index sets}]}{%
\ifthenelse{\equal{#1}{C}}{\item[\textbf{Parameters}]}{%
\ifthenelse{\equal{#1}{D}}{\item[\textbf{State variables}]}{%
\ifthenelse{\equal{#1}{E}}{\item[\textbf{Stochastic variables}]}{%
\ifthenelse{\equal{#1}{O}}{\item[\textbf{Other}]}{}}}}}}
}

\setlength{\nomlabelwidth}{1.5cm}
\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{A}{SDP sets}{%
  \ifstrequal{#1}{B}{Index sets}{%
  \ifstrequal{#1}{C}{Parameters}{%
  \ifstrequal{#1}{E}{Stochastic variables}{%
  \ifstrequal{#1}{D}{Decision variables}{%
  \ifstrequal{#1}{O}{Other Symbols}{}}}}}}%
]}

%For sets
%\nomenclature[A]{$\mathcal{T}_{Stage}$}{set of stages within the period}
\nomenclature[A]{$\mathcal{S}_{t}$}{set of state variables}
\nomenclature[A]{$\mathcal{S}_{s,t}$}{set of stochastic variables}
\nomenclature[A]{$\mathcal{S}_{p,t}$}{set of deciding variables}
%\nomenclature[A]{$\mathcal{N}_{State}$}{List of discrete }
%\nomenclature[A]{$\mathcal{N}_{Scen}$}{set of deciding variables}



\nomenclature[B]{$\mathcal{G}$}{Set of time steps within the stage}


%Stochastic variables
\nomenclature[E]{$\lambda^{Spot}_g$}{Electricity price from spot market in time step g [$\frac{NOK}{kWh}$]}
\nomenclature[E]{$P_{g}^{Inflex}$}{Inflexible load in the household in time step g [$kWh$]}
\nomenclature[E]{$\delta_g^{EV}$}{EV connected to building $\{0,1\}$}
\nomenclature[E]{$I_g^{Irr}$}{Irradiation on PV panels [$\frac{kWh}{m^2}$]}
\nomenclature[E]{$\delta_g^{Occ}$}{Occupancy presence $\{0,1\}$}
\nomenclature[E]{$T^{Out}$}{Daily average outdoor temperature [$\degree C$]}



%Decision variables
\nomenclature[D]{$p_g^{imp}, p_g^{exp}$}{Energy imported/exported to household [$\frac{kWh}{h}$]}
%\nomenclature[D]{$p_g^{exp}$}{Energy exported from household [$\frac{kWh}{h}$]}
\nomenclature[D]{$p^{peak}$}{Peak of imported energy [$\frac{kWh}{h}$]}
\nomenclature[D]{$\gamma$}{SOS-2 variables}

%Special variable
\nomenclature[D]{$C_{p^{peak},s^e_{t+1}}^{peak}$}{Expected future cost from peak power [$\frac{NOK}{\frac{kWh}{h}}$]}

%EV
\nomenclature[D]{$e_g^{soc}$}{State of charge for EV for time step t [$kWh$]}
\nomenclature[D]{$e_g^{ch}$}{Input power to EV for time step t [$\frac{kWh}{h}$]}

%BAT
\nomenclature[D]{$b_g^{soc}$}{State of charge for Battery for time step t [$kWh$]}
\nomenclature[D]{$b_g^{ch},b_t^{dch}$}{Input/output power to battery for time step t [$\frac{kWh}{h}$]}

%PV
\nomenclature[D]{$\theta_g^{prod}$}{Power produced from PV system [$\frac{kWh}{h}$]}

%Heat
\nomenclature[D]{$\mu_g^{indoor}$}{Indoor temperature of the building [$\degree C$]}
\nomenclature[D]{$\mu_g^{Heater}$}{Heater power usage for building heating [$\frac{kWh}{h}$]}
%\nomenclature[D]{$\mu_g^{\Delta T}$}{Change in energy in room [$\frac{kWh}{h}$]}

%Parameters

\nomenclature[C]{$C^{grid}$}{DSO energy tariff for imported energy [$\frac{NOK}{kWh}$]}
\nomenclature[C]{$P^{imp,max}$}{Maximum power import to building [$\frac{kWh}{h}$]}
\nomenclature[C]{$P_n^{Peak}$}{Peak power at point $n$ [$\frac{kWh}{h}$]}
\nomenclature[C]{$P_0^{Peak}$}{Initial peak power [$\frac{kWh}{h}$]}
\nomenclature[C]{$Tax$}{Value added tax for purchase of electricity [$p.u$]}



%EV
\nomenclature[C]{$E^{Cap}$}{EV storage capacity [$kWh$]}
\nomenclature[C]{$\eta^{EV,ch}$}{EV charging efficiency [$\%$]}
\nomenclature[C]{$E^{Max}$}{Maximum EV charging capacity [$kWh$]}
\nomenclature[C]{$E_g^{soc_{min}},E_g^{soc_{max}}$}{Min/Max EV soc capacity [$kWh$]}
\nomenclature[C]{$E^{Load}$}{EV load when not present at home [$kWh$]}
\nomenclature[C]{$E^{Start/Stop}$}{EV start/end soc [$kWh$]}

%HERE I AM, ONCE AGAIN!
%BAT
\nomenclature[C]{$B^{Cap}$}{Battery storage capacity [$kWh$]}
\nomenclature[C]{$\eta^{B,dch},\eta^{B,ch}$}{Discharge/charge efficiency for battery [$\%$]}
\nomenclature[C]{$B^{dch},B^{ch}$}{Discharge/charge capacity for battery [$\frac{kWh}{h}$]}
\nomenclature[C]{$B^{Start/Stop}$}{Battery start/end soc [$kWh$]}
\nomenclature[C]{$B^{Min},B^{Max}$}{Min/Max battery soc capacity [$kWh$]}

%PV
\nomenclature[C]{$A^{roof}$}{PV system area [$m^2$]}
\nomenclature[C]{$\eta^{PV}$}{Total efficiency for PV system [$\%$]}


%Heat
\nomenclature[C]{$M^{Heater}$}{Heater rated capacity [$\frac{kWh}{h}$]}
\nomenclature[C]{$M^{A}$}{Size of building floor area [$m^2$]}
\nomenclature[C]{$M^{T_{Set}}$}{Start/end temperature of the building [$\degree C$]}
\nomenclature[C]{$M_g^{T_{Down}},M_g^{T_{Up}}$}{Lower/upper temperature boundary [$\degree C$]}
\nomenclature[C]{$M^{Storage}$}{specific heat capacity for heating storage in building [$\frac{kWh}{m^2\cdot K}$]}
\nomenclature[C]{$\alpha_g^{HL}$}{Time-dependent heat loss constant [$kWh$]}
\nomenclature[C]{$\beta_g^{HL}$}{Time-dependent heat loss slope [$\frac{kWh}{\degree C}$]}
\nomenclature[C]{$M^{Occ}$}{Heat gained due to occupancy [$\frac{kWh}{h}$]}

\printnomenclature
%For parameters




\begin{align}
    & min \; [Import - Export + Future] \label{eq:Obj_function}\\
    & Import = \sum_{g \in \mathcal{G} } p_g^{imp}\cdot (C^{grid} + \lambda_g^{Spot})\cdot (1+Tax) \nonumber\\
    & Export = \sum_{g \in \mathcal{G} } p_g^{exp}\cdot \lambda_g^{Spot} \nonumber \\
    & Future =  C_{p^{peak},s_{t+1}^{e}}^{peak}   \nonumber
\end{align}
\begin{subequations}
    \begin{flalign}
        & p^{peak} \geq P_0^{Peak} \label{eq:Memory_power}\\
        & p^{peak} \geq p_g^{imp} \quad \forall g\in \mathcal{G} \label{eq:hourly_power}\\
        & C_{p^{peak},s_{t+1}^{e}}^{peak} =   \sum_{n \in \mathcal{N}_{State}} \gamma_n \cdot C_{P_n^{Peak},s_{t+1}^{e}}^{peak} \label{eq:SOS2_decision} \\
        & p^{peak} = \sum_{n \in \mathcal{N}_{State}} \gamma_n \cdot P_n^{Peak} \label{eq:SOS2_binding} \\
        & \sum_{n \in \mathcal{N}_{State}} \gamma_n = 1 \label{eq:SOS2_var}
    \end{flalign}
\end{subequations}
\begin{align}
    & p_g^{imp} - p_g^{exp} + \theta_g^{prod}  + b_g^{dch} = \nonumber \\
    & P_g^{Inflex} + e_g^{ch} + \mu_g^{Heater} + b_g^{ch} \cdot \eta^{B,ch} \quad \forall g \in \mathcal{G} \label{eq:Energy_balance}
\end{align}  
\begin{subequations}
    \begin{align}
    & e_g^{soc}-e_{g-1}^{soc} = e_g^{ch}\eta^{EV,ch}(\delta_g^{EV}) \nonumber \\
    & -E^{Load} (1-\delta_g^{EV}) \quad  \forall g \in \mathcal{G} \backslash g \neq 1 \label{eq:EV_soc_balance} \\
    & e_g^{soc} - E^{Start/Stop} = \nonumber \\
    & e_g^{ch} \eta^{EV,ch}-E^{Load}\cdot (1-\delta_g^{EV}) \quad g = 1 \label{eq:soc_balance_EV} \\
    & E^{Start/Stop} = e_g^{soc} \quad g = 24 \label{eq:soc_balance,init} \\
    & 0 \leq e_g^{ch} \leq E^{Max} \quad \forall g \in \mathcal{G} \label{eq:EV_charge_lim} \\
    & E_g^{soc,min} \leq e_g^{soc} \leq E_g^{soc,max} \quad \forall g \in \mathcal{G} \label{eq:EV_soc_lim} 
    \end{align}
\end{subequations}

\begin{subequations}
    \begin{align}
    & b_g^{soc} - b_{g-1}^{soc} = b_g^{ch} - \frac{b_g^{dch}}{\eta^{B,dch}} \quad \forall g \in \mathcal{G} \backslash g \neq 1 \label{eq:BAT_balance} \\
    & b_g^{soc} - B^{{Start/Stop}} = b_g^{ch} - \frac{b_g^{dch}}{\eta^{B,dch}} \quad g = 1 \label{eq:BAT_balance_init} \\
    & b_g^{soc} = B^{{Start/Stop}}  \quad g = 24 \label{eq:BAT_balance_end} \\
    & 0 \leq b_g^{ch} \leq B^{ch,max} \quad \forall g \in \mathcal{G} \label{eq:Bat_charge_lim} \\
    & 0 \leq b_g^{dch} \leq B^{dch,max} \quad \forall g \in \mathcal{G} \label{eq:Bat_discharge_lim} \\
    & B^{Min} \leq b_g^{soc} \leq B^{Max} \quad \forall g \in \mathcal{G} \label{eq:Bat_soc_lim} \\
    \end{align}
\end{subequations}

\begin{align}
    & \theta_g^{prod} = A^{roof} \cdot \eta^{PV}\cdot I_g^{Irr} \quad \forall g \in \mathcal{G} \label{eq:PV_prod} 
\end{align}

\begin{subequations}
    \begin{align}
    & \mu_g^{Heater} + M^{Occ}\cdot \delta_g^{Occ} = \mu_g^{\Delta T} + M^{HL}_g \quad \forall g \in \mathcal{G} \label{eq:Heat_balance} \\ 
    & \mu_g^{\Delta T} = M^{A} M^{soc} (\mu_g^{indoor} - \mu_{g-1}^{indoor}) \; \forall g \in \mathcal{G} \backslash g \neq 1 \\
    & \mu_g^{\Delta T} = M^{A} M^{soc} (\mu_g^{indoor} - M^{T_{Set}}) \quad g = 1 \\
    & \mu_g^{indoor} = M^{T_{Set}} \quad g = 24 \label{eq:Heat_balance_end} \\
    & M^{HL}_t = \alpha_g^{HL} + \beta_g^{HL}\cdot T^{Out}  \quad \forall g \in \mathcal{G} \label{eq:HL} \\
    & 0 \leq \mu_g^{Heater} \leq M^{Rated} \quad \forall g \in \mathcal{G} \label{eq:Heater} \\
    & M_g^{T_{Down}} \leq \mu_g^{indoor} \leq M_g^{T_{Up}} \quad \forall g \in \mathcal{G} \label{eq:Heat_lim_empty}
    \end{align}
    \label{eq:heat}
\end{subequations}


The second suggested tariff, measured peak, is on the contrary to subscribed capacity straightforward to implement (with smart meters) and exists for many commercial/industrial customers today. It is fairly understandable, also for passive end-users, and capacity is priced directly without any action required on forehand. Costs are also fairly predictable, which translates to stable incomes for the DSOs. However, there are significant drawbacks of this tariff. With costs being based on monthly peaks, a very high peak early in the month removes all incentives to reduce peaks for the rest of the month. Therefore, peaks can be hard to predict and can happen somewhat randomly. Thus, a methodology to predict peaks and plan for it is required. Advantages and drawbacks of both the two grid tariff structures are presented in \Cref{tariffadvantages}.

\begin{table}[h]

\begin{tabular}{lcc}
                                        & \multicolumn{1}{l}{\textbf{Measured peak}}                                                                         & \multicolumn{1}{l}{\textbf{Subscribed capacity}}                                                  \\ \hline
\multicolumn{1}{c}{\textbf{Advantages}} & \begin{tabular}[c]{@{}c@{}}1) Easy to implement\\ 2) Easy to understand\\ 3) Predictable costs\end{tabular}           & \begin{tabular}[c]{@{}c@{}}1) Predictable costs\\ 2) Incentivizes\\ active customers\end{tabular} \\ \hline
\textbf{Drawbacks}                      & \begin{tabular}[c]{@{}c@{}}1) Early peaks removes\\ peak shaving incentives\\ 2) Hard to predict peak\end{tabular} & \begin{tabular}[c]{@{}c@{}}1) Hard to implement\\ 2) Hard to understand\end{tabular}              \\ \hline
\end{tabular}
\caption{Advantages and drawbacks of measured peak and subscribed capacity grid tariff structures.}
\label{tariffadvantages}
\end{table}


\newpage
hello
\newpage

\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}



Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,references}


\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

